Polynomial Interrupt Timed Automata

Interrupt Timed Automata (ITA) form a subclass of stopwatch automata where reachability and some variants of timed model checking are decidable even in presence of parameters. They are well suited to model and analyze real-time operating systems. Here we extend ITA with polynomial guards and updates, leading to the class of polynomial ITA (PolITA). We prove the decidability of the reachability and model checking of a timed version of CTL by an adaptation of the cylindrical decomposition method for the first-order theory of reals. Compared to previous approaches, our procedure handles parameters and clocks in a unified way. Moreover, we show that PolITA are incomparable with stopwatch automata. Finally additional features are introduced while preserving decidability.

==> macros.tex <==
\makeatletter
%% Lettres fr\'equentes
%%% Fonctions d'ordre sup\'erieur
\newcommand{\m@ken@medcal}[2][\@error]{\expandafter\def\csname #1\endcsname{\ensuremath{\mathcal{#2}}}}
\newcommand{\m@kecal}{\@dblarg\m@ken@medcal}
\newcommand{\m@ken@medbb}[2][\@error]{\expandafter\def\csname #1\endcsname{{\ensuremath{\mathbb{#2}}}}}
\newcommand{\m@kebb}{\@dblarg\m@ken@medbb}
\newcommand{\m@ken@medsf}[2][\@error]{\expandafter\def\csname #1\endcsname{{\ensuremath{\mathsf{#2}}}}}
\newcommand{\m@kesf}{\@dblarg\m@ken@medsf}
\newcommand{\m@ken@medmathtxt}[2][\@error]{\expandafter\def\csname #1\endcsname{{\ensuremath{\textit{#2}}}}}
\newcommand{\m@kemathtxt}{\@dblarg\m@ken@medmathtxt}
%%% CALigraphiques
\m@kecal{A}
\m@kecal{T}
\m@kecal[Lang]{L}
\m@kecal[Cs]{C}
\m@kecal{U}
\m@kecal[Dc]{D}
\m@kecal[Reg]{R}
\m@kecal{P}
\m@kecal{S}

%%% Black-Board
\m@kebb{N}
\m@kebb{Z}
\m@kebb{Q}
\m@kebb{R}
\m@kebb{C}
\m@kebb{D}
\m@kebb{F}
\m@kebb{K}
\m@kebb[An]{A}

%%% Sans-s\'eriF
%\m@kesf[propp]{p}
\m@kesf{NP}
\m@kesf{coNP}
\m@kesf{NEXPSPACE}
\m@kesf{EXPSPACE}
\m@kesf{PSPACE}

%%% Texte (italic) dans des math
\m@kemathtxt{Poly}
\m@kemathtxt[timeSuc]{succ}
\m@kemathtxt{sign}
\m@kemathtxt{Run}
%%% Autres

\newcommand{\mmid}{\:\middle|\:}
\newcommand{\eps}{\varepsilon}
\newcommand{\fee}{\varphi}
\newcommand{\oneto}[1]{\left\{1,\dots,#1\right\}}
\newcommand{\zeroto}[1]{\left\{0,\dots,#1\right\}}
\newcommand{\tr}[1]{\xrightarrow{#1}}
\newcommand{\rel}{\bowtie}
\newcommand{\ita}{\textsc{ITA}\xspace}
\newcommand{\polita}{\textsc{PolITA}\xspace}
\newcommand{\swa}{\textsc{SWA}\xspace}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\CTL}{\textsf{CTL}\xspace}
\newcommand{\TCTL}{\textsf{TCTL}\xspace}
\newcommand{\TCTLint}{\textsf{TCTL}$_\textrm{int}$\xspace}
\newcommand{\until}{\ensuremath{{\sf \,U\,}}}
\newcommand{\always}{\ensuremath{{\sf A\,}}}
\newcommand{\expath}{\ensuremath{{\sf E\,}}}
\newcommand{\globally}{\ensuremath{{\sf G}}}
\newcommand{\eventually}{\ensuremath{{\sf F}}}
\newcommand{\timedtrans}[3]{%
  \begin{tabular}{c}
    \(#1\) \\ % Guarde
    \(#2\) \\ % Lettre
    \(#3\) % Resets
  \end{tabular}
}
\newcommand{\timedtransnoreset}[2]{%
  \begin{tabular}{c}
    \(#1\) \\ % Guarde
    \(#2\)    % Lettre
  \end{tabular}
}
\newcommand{\derive}[2]{\frac{\partial #1}{\partial #2}}

\makeatother
